Consistency of Constrained Spectral Clustering under Graph Induced Fair Planted Partitions

Spectral clustering is popular among practitioners and theoreticians alike. While performance guarantees for spectral clustering are well understood, recent studies have focused on enforcing ``fairness'' in clusters, requiring them to be ``balanced'' with respect to a categorical sensitive node attribute (e.g. the race distribution in clusters must match the race distribution in the population). In this paper, we consider a setting where sensitive attributes indirectly manifest in an auxiliary \textit{representation graph} rather than being directly observed. This graph specifies node pairs that can represent each other with respect to sensitive attributes and is observed in addition to the usual \textit{similarity graph}. Our goal is to find clusters in the similarity graph while respecting a new individual-level fairness constraint encoded by the representation graph. We develop variants of unnormalized and normalized spectral clustering for this task and analyze their performance under a \emph{fair} planted partition model induced by the representation graph. This model uses both the cluster membership of the nodes and the structure of the representation graph to generate random similarity graphs. To the best of our knowledge, these are the first consistency results for constrained spectral clustering under an individual-level fairness constraint. Numerical results corroborate our theoretical findings.

==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See \Cref{section:constraint} for the new fairness constraint, \Cref{section:unnormalized_repsc,section:normalized_repsc} for the algorithms, \Cref{section:rsbm} for the new random graph model, \Cref{section:consistency_results,section:discussion} for consistency results, and \Cref{section:numerical_results,appendix:additional_experiments} for numerical results.}
  \item Did you describe the limitations of your work?
    \answerYes{See \Crefrange{remark:spectral_relaxation}{remark:approximate_urepsc} where we discuss issues with spectral relaxation, computational complexity, and lack of theoretical guarantees for the approximate variant of our algorithms. Also see \Cref{section:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Our algorithms are intended to learn more ``fair'' clusters. While one can argue about the definition of fairness itself, within the context of this work, we do not see a negative societal impact if the algorithms are used as intended.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \Cref{assumption:R_is_d_regular} and \Cref{theorem:consistency_result_unnormalized,theorem:consistency_result_normalized}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See \Cref{section:proof_of_theorems}}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code submitted as supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See the description of experiments in \Cref{section:numerical_results}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{A careful look at the plots shows that error bars are present, though the variation is very small.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{The experiments were run on a standard desktop and did not require any specialized hardware.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We have added an appropriate reference for the FAO Trade Network. No code from outside sources was used.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
